Privacy-Preserving Visual Localization with Event Cameras

We consider the problem of client-server localization, where edge device users communicate visual data with the service provider for locating oneself against a pre-built 3D map. This localization paradigm is a crucial component for location-based services in AR/VR or mobile applications, as it is not trivial to store large-scale 3D maps and process fast localization on resource-limited edge devices. Nevertheless, conventional client-server localization systems possess numerous challenges in computational efficiency, robustness, and privacy-preservation during data transmission. Our work aims to jointly solve these challenges with a localization pipeline based on event cameras. By using event cameras, our system consumes low energy and maintains small memory bandwidth. Then during localization, we propose applying event-to-image conversion and leverage mature image-based localization, which achieves robustness even in low-light or fast-moving scenes. To further enhance privacy protection, we introduce privacy protection techniques at two levels. Network level protection aims to hide the entire user's view in private scenes using a novel split inference approach, while sensor level protection aims to hide sensitive user details such as faces with light-weight filtering. Both methods involve small client-side computation and localization performance loss, while significantly mitigating the feeling of insecurity as revealed in our user study. We thus project our method to serve as a building block for practical location-based services using event cameras. Project page including the code is available through this link: https://82magnolia.github.io/event\_localization/.

==> sec/a_user_study.tex <==


\subsection{User Study}
\label{sec:user_study}

% Along with the low-level and high-level analysis performed in Section~\ref{sec:network_eval} and ~\ref{sec:sensor_eval}, 
We conduct a user study to examine how people would feel about our privacy protection pipeline.
We request 39 volunteers to answer a survey that assesses how insecure people feel about various capturing scenarios, where the insecurity is scored from 1 to 5 with larger scores indicating higher insecurity.
As shown in Figure~\ref{fig:survey}, the survey first makes an assessment of being captured with normal cameras for various situations such as tourist spots and CCTV.
% As shown in Figure~\ref{fig:survey}a, the survey makes an initial assessment of being captured with normal cameras for situations such as tourist spots and CCTV.
Then the participants are asked about their feeling of insecurity with event cameras after seeing (1) raw event measurements, (2) image reconstructions from events, and (3) image reconstructions after network/sensor level protection.
% Then the survey evaluates event cameras in three steps: the users first observe raw event measurements, then the image reconstructions from events, and finally the image reconstructions after network/sensor level protection.
% We share the full survey along with the detailed answers of the subjects in Appendix~\ref{sec:supp_user_study}.

% Figure~\ref{fig:survey} displays the survey results.
In the initial assessment from Figure~\ref{fig:survey}-(a) people have varying levels of insecurity depending on the capturing scenario.
The averaged insecurity scores provide a rough translation cue for interpreting the scores obtained for event cameras and privacy protections.
In Figure~\ref{fig:survey}-(b), the subjects first give a low insecurity score when they see the raw events but increase their score once they observe that image reconstruction is possible.
The scores drop after people observe the sensor level protection results, to a level roughly equivalent to `being captured on CCTV / friend's camera'.
Furthermore, the scores are even lower for network level protection, as the scene content is completely hidden.
The results show that our method can indeed alleviate the concerns presented by users when using AR/VR services.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]
  {figures/fig_comments.pdf}
   \caption{Positive and negative comments from the user study about our privacy protection method.}
   \label{fig:comments}
   \vspace{-1em}

\end{figure}

\subsubsection{User Comments}
Along with the insecurity scoring, we requested the users to optionally leave comments about their evaluations.
We share the user comments in Figure~\ref{fig:comments}.
Overall, the positive comments emphasize the fact that for sensor level protection the facial details are sufficiently removed and for network level protection the reconstructions successfully hide the entire user's view.
Nevertheless, there were some negative comments about the sensor level protection that other signals such as unique gestures or body features are not obscured.
Devising a privacy protection method that can cover a wider range of biometric signals is left as future work.

